Strength in numbers: optimal and scalable combination of LHC new-physics searches

To gain a comprehensive view of what the LHC tells us about physics beyond the Standard Model (BSM), it is crucial that different BSM-sensitive analyses can be combined. But in general, search analyses are not statistically orthogonal, so performing comprehensive combinations requires knowledge of the extent to which the same events co-populate multiple analyses' signal regions. We present a novel, stochastic method to determine this degree of overlap and a graph algorithm to efficiently find the combination of signal regions with no mutual overlap that optimises expected upper limits on BSM-model cross-sections. The gain in exclusion power relative to single-analysis limits is demonstrated with models with varying degrees of complexity, ranging from simplified models to a 19-dimensional supersymmetric model.

==> cpcfront.tex <==
% A submitted program is expected to be of benefit to other physicists or physical chemists, or be an exemplar of good programming practice, or illustrate new or novel programming techniques which are of importance to some branch of computational physics or physical chemistry.
%
%Acceptable program descriptions can take different forms. The following Long Write-Up structure is a suggested structure but it is not obligatory. Actual structure will depend on the length of the program, the extent to which the algorithms or software have already been described in literature, and the detail provided in the user manual.
%
%Your manuscript and figure sources should be submitted through the Elsevier Editorial System (EES) by using the online submission tool at \\
%http://www.ees.elsevier.com/cpc.
%
%In addition to the manuscript you must supply: the program source code; job control scripts, where applicable; a README file giving the names and a brief description of all the files that make up the package and clear instructions on the installation and execution of the program; sample input and output data for at least one comprehensive test run; and, where appropriate, a user manual. These should be sent, via email as a compressed archive file, to the CPC Program Librarian at cpc@qub.ac.uk.
%

% Computer program descriptions should contain the following
% PROGRAM SUMMARY.

\noindent \textbf{PROGRAM SUMMARY H}

\begin{small}
\noindent
\emph{Program Title:} TACO                                      \\
\emph{Licensing provisions:} GPLv3                              \\
\emph{Programming language:} Python                             \\

%\emph{Supplementary material:} \\
% Fill in if necessary, otherwise leave out.
%\emph{Journal reference of previous version:}                  \\
  %Only required for a New Version summary, otherwise leave out.
%\emph{Does the new version supersede the previous version?:}   \\
  %Only required for a New Version summary, otherwise leave out.
%\emph{Reasons for the new version:}\\
  %Only required for a New Version summary, otherwise leave out.
%\emph{Summary of revisions:}*\\
  %Only required for a New Version summary, otherwise leave out.

\noindent \emph{Nature of problem:}\\ %(approx. 50-250 words)
With a decade of LHC operation having ruled out the most obvious models of BSM
physics, there is an increasing presumption that new physics will not be
discoverable via a single, powerful experimental signature, but will disperse
across many signatures at a level below direct exclusion in any one search
analysis. Definitive LHC statements about any dispersed signature hence require
combination of as many analyses as possible. But not all analyses \emph{can} be
combined: frequently, multiple useful analyses from a single experiment overlap
in their exploration of event topologies and phase-space, meaning that
%in a na\"ive dataset combination
event selections and observables may be double-counted. Such overlaps, and their
statistical significance, are impossible to identify purely from cut
lists alone. And when analysis overlaps \emph{are} known, there remains the
problem of identifying which compatible subset will place the optimal constraint
on a given BSM model. Scaling these identifications as required for LHC legacy
interpretations is a significant strategic problem.

\vspace{1ex}

\noindent \emph{Solution method:}\\ %(approx. 50-250 words)
To identify degrees of double-counting between analysis signal-regions (SRs), a
sampling over the minimal parameter spaces of \smodels simplified BSM-model
topologies is used to populate a full set of search SRs. We use a modified
version of the \MA analysis toolkit on events generated at these points to
produce a Poisson-bootstrapped family of SR expected event yields, and hence
estimate the SR overlaps; specifying an acceptable threshold in overlap coefficient
then defines a binary matrix of allowed and disallowed pairwise SR-combinations. From
this, SR combinations can be viewed as a directed acyclic graph, on which a
hierarchical weighted longest-path computation can be used to identify the best-expected SR
combination for limit-setting on any given BSM model.

\vspace{1ex}

\noindent \emph{Additional comments including Restrictions and Unusual
  features:}\\ %(approx. 50-250 words)
This work considers signal regions only, overlaps between signal regions
of one analysis and control regions of another analysis are not quantified.
Neither are background overlaps between different analyses: signal-estimated
overlaps are assumed representative of all events falling into a given
topological \& kinematic bin.

